Learning First-Order Symbolic Planning Representations That Are Grounded

Two main approaches have been developed for learning first-order planning (action) models from unstructured data: combinatorial approaches that yield crisp action schemas from the structure of the state space, and deep learning approaches that produce action schemas from states represented by images. A benefit of the former approach is that the learned action schemas are similar to those that can be written by hand; a benefit of the latter is that the learned representations (predicates) are grounded on the images, and as a result, new instances can be given in terms of images. In this work, we develop a new formulation for learning crisp first-order planning models that are grounded on parsed images, a step to combine the benefits of the two approaches. Parsed images are assumed to be given in a simple O2D language (objects in 2D) that involves a small number of unary and binary predicates like "left", "above", "shape", etc. After learning, new planning instances can be given in terms of pairs of parsed images, one for the initial situation and the other for the goal. Learning and planning experiments are reported for several domains including Blocks, Sokoban, IPC Grid, and Hanoi.

==> asp_encoding.tex <==
\section{ASP Encoding}

We solve the learning problem formulated above using answer set programming (ASP). This section presents the program whose answer sets correspond to solutions to this problem. The solutions are found by calling the ASP solver \textsc{clingo}\xspace \cite{torsten:asp,torsten:clingo} once for each iteration of incremental learning. Once a preference ordering on solutions is defined, some of these problems are shown to be solved \emph{optimally}, meaning that there is no simpler representation compatible with the input data.

\subsection{Program}

The ASP code  for learning the instances $P_i{=}\tup{D,I_i}$ from multiple input graphs $G_i$, using a pool of predicates $\sigma_k$ for some $k\in \mathbb{N}$, is shown in Figure~\ref{fig:program}. Each graph $G_i$ is assumed to be encoded using the atoms \atom|node(I,S)| and \atom|tlabel(I, T,L)| where \atom|S| and \atom|T=(S1,S2)| denote nodes and transitions
in the graph $G_i$ with index \atom|I|, and \atom|L| denotes the corresponding action label. At each step of incremental learning, each instance \atom|I| and node \atom|S| from this instance that must be taken into account at that step is marked with an atom \atom|relevant(I,S)|. Instances that are not relevant for this step are marked with \atom|disabled(I)|. Truth values \atom|V| of ground atoms \atom|(P,OO)| from the language $L_{\sigma_k}$, in the state \atom|S| of instance \atom|I|, are encoded in the input with atoms \atom|val(I,(P,OO),S,V)|. When computing the truth values for such atoms, \textit{redundant} predicates from $\sigma_k$ are pruned. A predicate is redundant when its denotation over all states in the training and test instances is the same as some previously considered predicate; i.e., given some enumeration of the predicates in the pool, the predicate $p_i$ is redundant iff there is $p_j$ such that for each state $s$ of each instance, $p^s_i = p^s_j$, $j<i$. Moreover, for each instance \atom|I|, we compute the predicates that are static over that instance, mark them with the fact \atom|f\_static(I,P)|, and encode their truth value \atom|V| in all states of that instance with a single fact \atom|val(I,(P,OO2),V)|. Each predicate \atom|P| in $\sigma_k$ is marked with the fact \atom|feature(P)|, and their arity \atom|N| is encoded by a fact \atom|f\_arity(P,N)|. Finally, for each domain, each \textit{object type} predicate \atom|P|  that has a non-empty denotation over the input instances is immediately selected as a predicate (via an atom \atom|pred(P)|) in order to allow the learned PDDL schemas to be typed. The number of action schemas is set to the number of action labels and the objects are extracted from the state valuations (\textbf{line 7}). The maximum number of predicates in $\lambda$ (the chosen set of predicates to define the learned domain) is set to the value of the constant \atom|num\_predicates| ($12$ by default). The maximum arity of an action is set to the value of the constant \atom|max\_arity| ($3$ by default). 

\begin{figure*}
\begin{Verbatim}[gobble=4,frame=single,numbers=left,codes={\catcode`$=3}]
    % Constants and options
    #const num_predicates = 12.
    #const max_action_arity = 3.
    
    % Define predicate arities with p_arity/2 
    nullary(F)   :- feature(F), f_arity(F,1), 1 \{ fval(I,(F,null_arg),0..1) \}.                
    nullary(F)   :- feature(F), f_arity(F,1), 1 \{ fval(I,(F,null_arg),S,0..1) : node(I,S) \}.  
    p_arity(F,N) :- feature(F), f_arity(F,N), not nullary(F).
    p_arity(F,0) :- nullary(F).
    :- p_arity(F,N), nullary(F), N > 0.
    
    % Actions and objects
    action(A) :- tlabel(I,(S,T),A), relevant(I,S).
    \{ a_arity(A,0..max_action_arity) \} = 1 :- action(A).
    object(I,O) :- not disabled(I), fval(I,(verum,(O,)),1).
    
    % Choose predicates from pool
    % Assumption: at least one argument O of a chosen predicate must be an object (i.e., O is not a shape)
    nelegible(F) :- fval(I,(F,(O,)),S,V), not object(I,O), O $\neq$ null.
    nelegible(F) :- fval(I,(F,(O,)),V), not object(I,O), O $\neq$ null.
    nelegible(F) :- fval(I,(F,(_,O)),V), not object(I,O).
    nelegible(F) :- fval(I,(F,(O,_)),V), not object(I,O).
    nelegible(F) :- fval(I,(F,(_,O)),S,V), not object(I,O).
    nelegible(F) :- fval(I,(F,(O,_)),S,V), not object(I,O).
    \{ pred(F) : feature(F), not nelegible(F) \} num_predicates.
    
    % Tuples of variables/constants for lifted effects and preconditions
    #defined constant/1.
    argtuple(null_arg,0). % Explicit zero arity predicates
    argtuple((C1,),1)     :- constant(C1).
    argtuple((V1,),1)     :- V1 = 1..max_action_arity.
    argtuple((C1,C2),2)   :- constant(C1), constant(C2).
    argtuple((C1,V2),2)   :- constant(C1), V2 = 1..max_action_arity.
    argtuple((V1,C2),2)   :- V1 = 1..max_action_arity, constant(C2).
    argtuple((V1,V2),2)   :- V1 = 1..max_action_arity, V2 = 1..max_action_arity.
    
    % Tuples of objects that ground the action schemas and atoms
    const_or_obj(I,O)             :- object(I,O).
    const_or_obj(I,O)             :- instance(I), constant(O).
    objtuple(I,null_arg,0)      :- instance(I). % Zero arity predicates
    objtuple(I,     (O1,),1)      :- object(I,O1), not constant(O1).
    objtuple(I,   (O1,O2),2)      :- object(I,O1), object(I,O2), not constant(O1), not constant(O2), O1 $\neq$ O2.
    objtuple(I,   (O1,O1),2)      :- object(I,O1), not constant(O1).
    constobjtuple(I, null_arg,0) :- instance(I). % Zero arity predicates
    constobjtuple(I,     (O1,),1) :- const_or_obj(I,O1).
    constobjtuple(I,   (O1,O2),2) :- const_or_obj(I,O1), const_or_obj(I,O2), O1 $\neq$ O2.
    constobjtuple(I,   (O1,O1),2) :- const_or_obj(I,O1).
    
    % Assumption: predicates have arity < 3
    :- p_arity(F,N), N > 2.
    
    % Mapping of lifted arguments for atoms into grounded arguments
    % Lifted atom is pair (P,T) where P is predicate and T is tuple of variables
    % and constants used to construct argument OO of grounded atom (P,OO).
    
    % for nullary actions
    map(I,(0,0,0,0),null_arg,null_arg,0)      :- instance(I).
    map(I,(0,0,0,0),(C,),(C,),1)              :- constobjtuple(I,(C,),1), constant(C).
    map(I,(0,0,0,0),(C1,C2),(C1,C2),2)        :- constobjtuple(I,(C1,C2),2), constant(C1), constant(C2).
    
    % for unary actions
    map(I,(O1,0,0,0),null_arg,null_arg,0)     :- objtuple(I,(O1,),1).
    map(I,(O1,0,0,0),(C,),(C,),1)             :- objtuple(I,(O1,),1), constobjtuple(I,(C,),1), constant(C).
    map(I,(O1,0,0,0),(1,),(O1,),1)            :- objtuple(I,(O1,),1).
    map(I,(O1,0,0,0),(C1,C2),(C1,C2),2)       :- objtuple(I,(O1,),1), constobjtuple(I,(C1,C2),2), constant(C1), constant(C2).
    map(I,(O1,0,0,0),(C,1),(C,O1),2)          :- objtuple(I,(O1,),1), constobjtuple(I,(C,O1),2), constant(C).
    map(I,(O1,0,0,0),(1,C),(O1,C),2)          :- objtuple(I,(O1,),1), constobjtuple(I,(O1,C),2), constant(C).
    
    % for actions of arity >= 2
    map(I,(O1,O2,0,0),null_arg,null_arg,0)    :- objtuple(I,(O1,O2),2).
    map(I,(O1,O2,0,0),(C,),(C,),1)            :- objtuple(I,(O1,O2),2), constobjtuple(I,(C,),1), constant(C).
    map(I,(O1,O2,0,0),(1,),(O1,),1)           :- objtuple(I,(O1,O2),2).
    map(I,(O1,O2,0,0),(2,),(O2,),1)           :- objtuple(I,(O1,O2),2).
    ...
    map(I,(0,0,O3,O4),(3,4),(O3,O4),2)        :- objtuple(I,(O3,O4),2), constobjtuple(I,(O3,O4),2).
    map(I,(0,0,O3,O4),(4,3),(O4,O3),2)        :- objtuple(I,(O3,O4),2), constobjtuple(I,(O4,O3),2).
    ...
    map(I,(0,O2,0,0),(2,),(O2,),1)            :- objtuple(I,(O2,),1).
    map(I,(0,0,O3,0),(3,),(O3,),1)            :- objtuple(I,(O3,),1).
    map(I,(0,0,0,O4),(4,),(O4,),1)            :- objtuple(I,(O4,),1).
    
    % Define variables used by actions
    % a_var(A,V): action A uses var V
    a_var(A,V) :- a_arity(A,N), V = 1..N.
    
    % Define variables appearing in a variable tuple
    t_var((V,),V)     :- argtuple((V,),1),    not constant(V), V $\neq$ null.
    t_var((V1,V2),V1) :- argtuple((V1,V2),2), not constant(V1).
    t_var((V1,V2),V2) :- argtuple((V1,V2),2), not constant(V2).
\end{Verbatim}
\vskip -1eM
\caption{The ASP code (part 1)}
\label{fig:program}
\end{figure*}


\begin{figure*}
\begin{Verbatim}[gobble=4,frame=single,numbers=left,codes={\catcode`$=3}]
    % An argtuple T is good for action A iff each V in T is an action var
    goodtuple(A,null_arg) :- action(A).
    goodtuple(A,T)    :- action(A), argtuple(T,N), a_var(A,V) : t_var(T,V).
    
    % Choice of lifted preconditions for actions
    % prec(A,M,V): atom M is negative (resp. positive) precondition of action A if V=0 (resp. V=1)
    \{ prec(A,(P,T),1) \}      :- action(A), pred(P), p_arity(P,N), argtuple(T,N), goodtuple(A,T).
    \{ prec(A,(P,T),0..1) \} 1 :- action(A), pred(P), p_arity(P,N), argtuple(T,N), goodtuple(A,T).
    
    % Choice of lifted effects for actions
    % eff(A,M,V): atom M is negative (resp. positive) effect of action A if V=0 (resp. V=1)
    p_static(P) :- pred(P), f_static(I,P) : instance(I).
    p_fluent(P) :- pred(P), not f_static(I,P) : instance(I).
    \{ eff(A,(P,T),0..1) \} 1 :- action(A), pred(P), not p_static(P), p_arity(P,N), argtuple(T,N), goodtuple(A,T).
    
    % Avoid noop actions and rule out contradictory effects
    :- action(A), \{ eff(A,(P,T),0..1) : pred(P), p_arity(P,N), argtuple(T,N) \} = 0.
    :- eff(A,M,0), eff(A,M,1).
    
    % Map graph edges to grounded actions
    
    % Factored applicability check. Defined for action arities up to 4
    % Static part 
    fappl(I,A,null_arg,null_arg)   :- instance(I), action(A), a_arity(A,0),
                                      fval(I,(P,OO),V)      : prec(A,(P,T),V), map(I,(0,0,0,0),T,OO,K), f_static(I,P).
    fappl(I,A,(1,),(O1,))          :- instance(I), action(A), a_arity(A,1), objtuple(I,(O1,),1),
                                      fval(I,(P,OO),V)      : prec(A,(P,T),V), map(I,(O1,0,0,0),T,OO,K), f_static(I,P).
    fappl(I,A,(1,2),(O1,O2))       :- instance(I), action(A), a_arity(A,N), N >= 2, objtuple(I,(O1,O2),2),
                                      fval(I,(P,OO),V)      : prec(A,(P,T),V), map(I,(O1,O2,0,0),T,OO,K), f_static(I,P).
    ...
    fappl(I,A,(3,4),(O3,O4))       :- instance(I), action(A), a_arity(A,N), N >= 4, objtuple(I,(O3,O4),2),
                                      fval(I,(P,OO),V)      : prec(A,(P,T),V), map(I,(0,0,O3,O4),T,OO,K), f_static(I,P).
    % Dynamic part
    fappl(I,A,null_arg,null_arg,S) :- instance(I), action(A), a_arity(A,0), relevant(I,S),
                                      fappl(I,A,null_arg,null_arg),
                                      fval(I,(P,OO),S,V)    : prec(A,(P,T),V), map(I,(0,0,0,0),T,OO,K), not f_static(I,P).
    
    fappl(I,A,(1,),(O1,),S)        :- instance(I), action(A), a_arity(A,1), objtuple(I,(O1,),1), relevant(I,S),
                                      fappl(I,A,(1,),(O1,)),
                                      fval(I,(P,OO),S,V)    : prec(A,(P,T),V), map(I,(O1,0,0,0),T,OO,K), not f_static(I,P).
    
    fappl(I,A,(1,2),(O1,O2),S)     :- instance(I), action(A), a_arity(A,N), N >= 2, objtuple(I,(O1,O2),2), relevant(I,S),
                                      fappl(I,A,(1,2),(O1,O2)),
                                      fval(I,(P,OO),S,V)    : prec(A,(P,T),V), map(I,(O1,O2,0,0),T,OO,K), not f_static(I,P).
    ...
    fappl(I,A,(3,4),(O3,O4),S)     :- instance(I), action(A), a_arity(A,N), N >= 4, objtuple(I,(O3,O4),2), relevant(I,S),
                                      fappl(I,A,(3,4),(O3,O4)),
                                      fval(I,(P,OO),S,V)    : prec(A,(P,T),V), map(I,(0,0,O3,O4),T,OO,K), not f_static(I,P).
    
    % Match edges with grounded actions
    % Factored next
    
    % Assumption: each edge (S1,S2) is labeled with unique action A, and maps to unique grounded action A(OO)
    :- tlabel(I,(S1,S2),A), tlabel(I,(S1,S2),B), A $\neq$ B.
    
    % fnext(I,K,O,S1,S2) : for edge tlabel(I,(S1,S2),A), K-th argument of A(OO) is object O
    
    % 1.a. Choose next S2 if ground action A(OO) is applicable in S1
      \{ fnext(I,0,0,  S1,S2) : tlabel(I,(S1,S2),A) \} = 1 :- action(A), a_arity(A,0), relevant(I,S1),
                                                            fappl(I,A,null_arg,null_arg,S1).
      \{ fnext(I,1,O1, S1,S2) : tlabel(I,(S1,S2),A) \} = 1 :- action(A), a_arity(A,1), relevant(I,S1),
                                                            fappl(I,A,(1,),(O1,),S1).
    1 \{ fnext(I,1,O1, S1,S2) : tlabel(I,(S1,S2),A) \}     :- action(A), a_arity(A,2), relevant(I,S1),
                                                            fappl(I,A,(1,2),(O1,O2),S1).
    1 \{ fnext(I,2,O2, S1,S2) : tlabel(I,(S1,S2),A) \}     :- action(A), a_arity(A,2), relevant(I,S1),
                                                            fappl(I,A,(1,2),(O1,O2),S1).
    ...
    1 \{ fnext(I,4,O4, S1,S2) : tlabel(I,(S1,S2),A) \}     :- action(A), a_arity(A,4), relevant(I,S1),
                                                            fappl(I,A,(1,2),(O1,O2),S1), fappl(I,A,(1,3),(O1,O3),S1),
                                                            fappl(I,A,(1,4),(O1,O4),S1), fappl(I,A,(2,3),(O2,O3),S1), 
                                                            fappl(I,A,(2,4),(O2,O4),S1), fappl(I,A,(3,4),(O3,O4),S1).
    
    % 1.b. If k1 -> O1 in (S1,S2), then k2 -> O2 in (S1,S2), for some O2, for each arg k1 of action A 
    % (i.e, A(OO) must be fully defined for (S1,S2))
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N), fnext(I,K1,O1,S1,S2), K1 > 0, K2 = 1..N, K2 $\neq$ K1,
       not fnext(I,K2,O2,S1,S2) : object(I,O2).
    
    % 1.c. It cannot be fnext(I,K,O1,S1,S2) and fnext(I,K,O2,S1,S2) with O1 < O2
    :- relevant(I,S1), fnext(I,K,O1,S1,S2), fnext(I,K,O2,S1,S2), O1 < O2.
    
    % 1.d. A(OO) cannot be mapped to two edges (S1,S2) and (S1,S3) with S2 < S3
    :- relevant(I,S1), tlabel(I,(S1,S2),A), tlabel(I,(S1,S3),A), S2 < S3, a_arity(A,0).
    :- relevant(I,S1), tlabel(I,(S1,S2),A), tlabel(I,(S1,S3),A), S2 < S3, a_arity(A,N), N >= 1, f
       next(I,1,O,S1,S2), fnext(I,1,O,S1,S3), not diff_fnext(I,A,K2,S1,S2,S3) : K2 = 2..N.
    diff_fnext(I,A,K,S1,S2,S3) :- relevant(I,S1), tlabel(I,(S1,S2),A), tlabel(I,(S1,S3),A), S2 < S3, a_arity(A,N), 
       N >= 1, K = 2..N, fnext(I,K,O1,S1,S2), fnext(I,K,O2,S1,S3), O1 $\neq$ O2.
    % 1.e. If tlabel(I,(S1,S2),A), then fnext(I,0,0,S1,S2) or fnext(I,1,_,S1,S2)
    :- relevant(I,S1), tlabel(I,(S1,S2),A), not fnext(I,0,0,S1,S2), not fnext(I,1,O,S1,S2) : object(I,O).
\end{Verbatim}
\vskip -1eM
\caption{The ASP code (part 2)}
\label{fig:program}
\end{figure*}


\begin{figure*}
\begin{Verbatim}[gobble=4,frame=single,numbers=left,codes={\catcode`$=3}]
    % 2. Check application of effects
    
    % 2.a. If A(OO1) mapped to (S1,S2) and eff(A,(P,OO2),V), then fval(I,(P,OO2),S2,V)
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,0),         fnext(I,0,0,S1,S2),                         eff(A,(P,T),V), map(I,(0,0,0,0),T,OO,K),   not f_static(I,P), fval(I,(P,OO),S2,1-V).
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,1),         fnext(I,1,O1,S1,S2),                        eff(A,(P,T),V), map(I,(O1,0,0,0),T,OO,K),  not f_static(I,P), fval(I,(P,OO),S2,1-V).
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N), N >= 2, fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2),   eff(A,(P,T),V), map(I,(O1,O2,0,0),T,OO,K), not f_static(I,P), fval(I,(P,OO),S2,1-V).
    ...
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N), N >= 4, fnext(I,3,O3,S1,S2), fnext(I,4,O4,S1,S2),   eff(A,(P,T),V), map(I,(0,0,O3,O4),T,OO,K), not f_static(I,P), fval(I,(P,OO),S2,1-V).
    
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,0),         fnext(I,0,0,S1,S2),                         eff(A,(P,T),V), map(I,(0,0,0,0),T,OO,K),       f_static(I,P), fval(I,(P,OO),1-V).
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,1),         fnext(I,1,O1,S1,S2),                        eff(A,(P,T),V), map(I,(O1,0,0,0),T,OO,K),      f_static(I,P), fval(I,(P,OO),1-V).
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N), N >= 2, fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2),   eff(A,(P,T),V), map(I,(O1,O2,0,0),T,OO,K),     f_static(I,P), fval(I,(P,OO),1-V).
    ...
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N), N >= 4, fnext(I,3,O3,S1,S2), fnext(I,4,O4,S1,S2),   eff(A,(P,T),V), map(I,(0,0,O3,O4),T,OO,K),     f_static(I,P), fval(I,(P,OO),1-V).
    
    % 2.b. If A(OO1) mapped to (S1,S2), fval(I,(P,OO2),S1,V) and fval(I,(P,OO2),S2,1-V), then eff(A,(P,OO2),1-V).
    :- relevant(I,S1), tlabel(I,(S1,S2),A),
       pred(P), fval(I,(P,null_arg),S1,V), fval(I,(P,null_arg),S2,1-V),
       not eff(A,(P,null_arg),1-V).
    
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N),
       pred(P), fval(I,(P,OO),S1,V), fval(I,(P,OO),S2,1-V), constobjtuple(I,OO,1),
       not eff(A,(P,T),1-V) : map(I,(0,0,0,0),T,OO,1),                        N >= 0;
       not eff(A,(P,T),1-V) : map(I,(O1,0,0,0),T,OO,1),  fnext(I,1,O1,S1,S2), N >= 1;
       not eff(A,(P,T),1-V) : map(I,(0,O2,0,0),T,OO,1),  fnext(I,2,O2,S1,S2), N >= 2;
       not eff(A,(P,T),1-V) : map(I,(0,0,O3,0),T,OO,1),  fnext(I,3,O3,S1,S2), N >= 3;
       not eff(A,(P,T),1-V) : map(I,(0,0,0,O4),T,OO,1),  fnext(I,4,O4,S1,S2), N >= 4.
    
    :- relevant(I,S1), tlabel(I,(S1,S2),A), a_arity(A,N),
       pred(P), fval(I,(P,OO),S1,V), fval(I,(P,OO),S2,1-V), constobjtuple(I,OO,2),
       not eff(A,(P,T),1-V) : map(I,(0,0,0,0),T,OO,2),                                             N >= 0;
       not eff(A,(P,T),1-V) : map(I,(O1,0,0,0),T,OO,2),  fnext(I,1,O1,S1,S2),                      N >= 1;
       not eff(A,(P,T),1-V) : map(I,(O1,O2,0,0),T,OO,2), fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2), N >= 2;
       not eff(A,(P,T),1-V) : map(I,(O1,0,O3,0),T,OO,2), fnext(I,1,O1,S1,S2), fnext(I,3,O3,S1,S2), N >= 3;
       not eff(A,(P,T),1-V) : map(I,(0,O2,O3,0),T,OO,2), fnext(I,2,O2,S1,S2), fnext(I,3,O3,S1,S2), N >= 3;
       not eff(A,(P,T),1-V) : map(I,(O1,0,0,O4),T,OO,2), fnext(I,1,O1,S1,S2), fnext(I,4,O4,S1,S2), N >= 4;
       not eff(A,(P,T),1-V) : map(I,(0,O2,0,O4),T,OO,2), fnext(I,2,O2,S1,S2), fnext(I,4,O4,S1,S2), N >= 4;
       not eff(A,(P,T),1-V) : map(I,(0,0,O3,O4),T,OO,2), fnext(I,3,O3,S1,S2), fnext(I,4,O4,S1,S2), N >= 4.
    
    % 3. Check application of applicable ground actions
    :- a_arity(A,2), fappl(I,A,(1,2),(O1,O2),S1),
       not fnext(I,2,O2,S1,S2) : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2).
    
    :- a_arity(A,3), fappl(I,A,(1,2),(O1,O2),S1), fappl(I,A,(1,3),(O1,O3),S1), fappl(I,A,(2,3),(O2,O3),S1),
       not fnext(I,3,O3,S1,S2) : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2).
    
    :- a_arity(A,4), fappl(I,A,(1,2),(O1,O2),S1), fappl(I,A,(1,3),(O1,O3),S1), fappl(I,A,(1,4),(O1,O4),S1), 
    fappl(I,A,(2,3),(O2,O3),S1), fappl(I,A,(2,4),(O2,O4),S1), fappl(I,A,(3,4),(O3,O4),S1),
       not fnext(I,4,O4,S1,S2) : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2), fnext(I,3,O3,S1,S2).
    
    % Fundamental constraints
    
    % F1. If (S1,S2) has label A, then A(OO) maps S1 to S2 for some object tuple OO
    :- relevant(I,S1), a_arity(A,0), X = \{ tlabel(I,(S1,S2),A) : node(I,S2) \}, 
       #count \{             S2 : tlabel(I,(S1,S2),A), fnext(I,0,0,S1,S2) \} $\neq$ X.
    :- relevant(I,S1), a_arity(A,1), X = \{ tlabel(I,(S1,S2),A) : node(I,S2) \}, 
       #count \{          O1,S2 : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2) \} $\neq$ X.
    :- relevant(I,S1), a_arity(A,2), X = \{ tlabel(I,(S1,S2),A) : node(I,S2) \}, 
       #count \{       O1,O2,S2 : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2) \} $\neq$ X.
    :- relevant(I,S1), a_arity(A,3), X = \{ tlabel(I,(S1,S2),A) : node(I,S2) \}, 
       #count \{    O1,O2,O3,S2 : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2), fnext(I,3,O3,S1,S2) \} $\neq$ X.
    :- relevant(I,S1), a_arity(A,4), X = \{ tlabel(I,(S1,S2),A) : node(I,S2) \}, 
       #count \{ O1,O2,O3,O4,S2 : tlabel(I,(S1,S2),A), fnext(I,1,O1,S1,S2), fnext(I,2,O2,S1,S2), fnext(I,3,O3,S1,S2), 
       fnext(I,4,O4,S1,S2) \} $\neq$ X.
    
    % F2. Different nodes are different states with respect to chosen predicates
    :- relevant(I,S1), relevant(I,S2), S1 < S2, fval(I,(P,OO),S2,V) : fval(I,(P,OO),S1,V), pred(P), not f_static(I,P).
\end{Verbatim}
\vskip -1eM
\caption{The ASP code (part 3)}
\label{fig:program}
\end{figure*}

==> planning.tex <==



==> preliminaries.tex <==
\section{Preliminaries}

%A (classical) planning instance is a pair $P\,{=}\,\tup{D,I}$ where $D$ is a first-order planning domain and $I$ represents the {instance information}. The planning domain $D$ contains a set of predicate symbols and a set of action schemas with preconditions and effects given by atoms $p(x_1, \ldots, x_k)$ or their negations, where $p$ is a domain predicate and each $x_i$ is a variable representing one of the arguments of the action schema. The instance information is a tuple $I\,{=}\,\tup{O,Init,Goal}$ where $O$ is a (finite) set of object names $c_i$, and $Init$ and $Goal$ are sets of ground atoms $p(c_1, \ldots, c_k)$ or their negations.

A planning problem $P\,{=}\,\tup{D,I}$ defines a \emph{labeled} graph $G(P)\,{=}\,\tup{V,E,L}$
where the nodes $n$ in $V$ correspond to the states $s(n)$ over $P$, and there is an edge $(n,n')$ in $E$ with label $a\in L$, if the state transition $(s(n),s(n'))$ is enabled by a ground instance of the schema $a$ in $P$. The states $s(n)$ are maximally consistent sets of ground literals over $P$ that comply with: $Init$ corresponds to
state $s(n_0)$ for some node $n_0$, states $s(n)$ and $s(n')$ are different if $n \not= n'$, and $(s(n),s(n'))$ is enabled by a ground action iff the preconditions of the action are true in $s(n)$, the effects are true in $s(n')$, and literals whose complements are not made true by the action have the same value in $s(n)$ and $s(n')$. The (partial) transition function associated with graph $G$, denoted by $f^G$, is given by: $f
^G(s,a)=s'$ iff $(n,n')\in E$ and $L((n,n'))=a$.

Given a suitable graphical representation, each state $s(n)$ of a planning problem can be associated with an image as well. This image may be \emph{parsed} in a number of ways. A common approach is to parse it into a set of \textit{object types} present in the image along with \textit{bounding boxes} indicating the position and size of every instance of each object type, as done in object recognition. Other visual information may be extracted as well, such as the \textit{geometric shape} of each object. We assume a parsing of this kind, and define the \textit{parsed image} of state $s(n)$, denoted by $im(n)$, as the set of triples $\{\tup{type(c),bb(c),shape(c)} \mid c \text{ is an object in } s(n)\}$, indicating the type, minimum bounding box, and shape of each object $c$ in $s(n)$. Each bounding box $bb(c)$ will be represented by its corner points $(x^{max}_{c},x^{min}_c,y^{max}_{c},y^{min}_{c})$.

==> representation_languages.tex <==
\section{Parsed Images: O2D Language}


*** Given a suitable graphical representation, each state $s(n)$ of a planning problem can be associated with an image as well. This image may be \emph{parsed} in a number of ways. A common approach is to parse it into a set of \textit{object types} present in the image along with \textit{bounding boxes} indicating the position and size of every instance of each object type, as done in object recognition. Other visual information may be extracted as well, such as the \textit{geometric shape} of each object. We assume a parsing of this kind, and define the \textit{parsed image} of state $s(n)$, denoted by $im(n)$, as the set of triples $\{\tup{type(c),bb(c),shape(c)} \mid c \text{ is an object in } s(n)\}$, indicating the type, minimum bounding box, and shape of each object $c$ in $s(n)$. Each bounding box $bb(c)$ will be represented by its corner points $(x^{max}_{c},x^{min}_c,y^{max}_{c},y^{min}_{c})$.

\label{sec:o2d_language} 

We introduce a family of languages for describing states represented as parsed images. We call such languages O2D (\textit{Objects in 2D space}). An O2D language is a first-order language whose predicates get their meanings from spatial properties and spatial relations defined directly over $im(s)$. I.e., the meaning of the predicates is \textit{grounded} in images. The defined languages include five binary relations, depicted in Figure \ref{fig:rels}. Four of them represent spatial relations encoding adjacency, overlap and relative size, while the fifth one relates objects to their shapes. The first-order signature $\sigma=(\mathcal{O},\mathcal{C},\mathcal{R})$ of an O2D language consists of \textit{constants} $\mathcal{O}=\{c_1,\dots,c_k\}$ for objects and their shapes; \textit{unary predicates} $\mathcal{
C}=\{\text{type}_1,\dots,\text{type}_n\}$ for object types; and \textit{binary predicates} $\mathcal{
R}=\{\text{left-of},\text{below-of},\text{overlaps-with},\text{smaller-than}$,$\text{shape}\}$. Given an O2D signature $\sigma$, we denote by $\mathcal{L}_\sigma$ the O2D language consisting only of atomic formulas over $\sigma$. Given a state $s$ with corresponding parsed image $\{\tup{type(c),bb(c),shape(c)} \mid c \text{ is an object in } s\}$, the interpretation of the O2D predicates in $s$ is as follows: 
\begin{itemize}
    \item $\text{type}^s_i \coloneqq \{ c \mid type(c) = type_i\}$, for $i=1,\dots,n$.
    \item $\text{left-of}^s \coloneqq \{(c,d) \mid x^{max}_{c} = x^{min}_{d}, \exists z: y^{min}_{d} < z < y^{max}_{d}, y^{min}_{c} < z < y^{max}_{c}\}$.
    \item $\text{below-of}^s \coloneqq \{(c,d) \mid y^{max}_{c} = y^{min}_{d}, \exists z: x^{min}_{d} < z < x^{max}_{d}, x^{min}_c < z < x^{max}_{c}\}$.
    \item $\text{overlaps-with}^s \coloneqq \{(c,d) \mid \exists z, z': x^{min}_c < z < x^{max}_{c}, x^{min}_{d} < z < x^{max}_{d}, y^{min}_{c} < z' < y^{max}_{c}, y^{min}_{d} < z' < y^{max}_{d}\}$.
    \item $\text{smaller-than}^s \coloneqq \{(c,d) \mid bb(c) \text{ is smaller than } bb(d)\}$.
    \item $\text{shape}^s \coloneqq \{(c,h) \mid shape(c)=h\}$.
\end{itemize}
Figure \ref{fig:blocks} illustrates the relationship between a state image and its O2D representation. The left side of the figure shows the image of a Blocksworld state $s$, generated with PDDLGym's graphical representation \cite{silver2020pddlgym}. The right side lists some of the ground O2D atoms in $\sigma(s)$, for the language whose signature $\sigma$ has constants $\mathcal{O}=\{r,t,b_0,\dots,b_6\}$ for the robot ($r$), table ($t$) and the blocks ($b_i$), and object types $\mathcal{C}=\{robot, block, table\}$.  For a state $s$, we denote by $\sigma(s)$ the representation of $s$ given by $\mathcal{L}_\sigma$, i.e., the set of all ground literals from $\mathcal{L}_\sigma$ that are true in $s$. 

\begin{figure}
    \centering
     \begin{subfigure}[b]{0.1\textwidth}
          \centering
          \resizebox{1\linewidth}{!}{
          \begin{tikzpicture}[every node/.style={minimum size=0.5cm-\pgflinewidth, outer sep=0pt}, background rectangle/.style={fill=gray!45}, show background rectangle]
            \draw[step=0.1cm,color=white] (0,0) grid (1.5,1.5);
            \node[fill=green] at (0.75,0.75) {};
            \node[fill=green!30] at (1.25,0.75) {};
        \end{tikzpicture}
          }
    \caption*{\text{left-of}}
     \end{subfigure}
     \begin{subfigure}[b]{0.1\textwidth}
          \centering
          \resizebox{1\linewidth}{!}{
            \begin{tikzpicture}[every node/.style={minimum size=0.5cm-\pgflinewidth, outer sep=0pt},, background rectangle/.style={fill=gray!45}, show background rectangle]
                \draw[step=0.1cm,color=white] (0,0) grid (1.5,1.5);
                \node[fill=green] at (0.75,0.75) {};
                \node[fill=green!30] at (0.75,1.25) {};
            \end{tikzpicture}
          } 
          \caption*{\text{below-of}}
     \end{subfigure}
      \begin{subfigure}[b]{0.1\textwidth}
      \centering
      \resizebox{1\linewidth}{!}{
        \begin{tikzpicture}[every node/.style={minimum size=0.5cm-\pgflinewidth, outer sep=-2pt},, background rectangle/.style={fill=gray!45}, show background rectangle]
            \draw[step=0.1cm,color=white] (0,0) grid (1.5,1.5);
            \node[fill=green] at (0.75,0.75) {};
            \node[fill=green!30] at (0.85,0.65) {};
        \end{tikzpicture}
      }
      \caption*{\text{overlaps-with}}
     \end{subfigure}
     
     
      \begin{subfigure}[b]{0.1\textwidth}
      \centering
      \resizebox{1\linewidth}{!}{
        \begin{tikzpicture}[every node/.style={minimum size=0.5cm-\pgflinewidth, outer sep=0pt},, background rectangle/.style={fill=gray!45}, show background rectangle]
            \draw[step=0.1cm,color=white] (0,0) grid (1.5,1.5);
            \node[fill=green,scale=0.58] at (0.75,0.75) {};
            \node[fill=green!30] at (1.25,0.75) {};
        \end{tikzpicture}
      }  
      \caption*{\text{smaller-than}}
     \end{subfigure}
    \begin{subfigure}[b]{0.1\textwidth}
      \centering
      \resizebox{1\linewidth}{!}{
        \begin{tikzpicture}[every node/.style={minimum size=0.27mm, inner sep=0mm, outer sep=0pt},, background rectangle/.style={fill=gray!45}, show background rectangle]
            \draw[step=0.1cm,color=white] (0,0) grid (1.5,1.5);
            \node[fill=green,scale=0.9] at (0.75,0.75) {\large$\bigcirc$};
            \node[fill=green,scale=0.85] at (1.15,1.15) {\Huge$\star$};
        \end{tikzpicture}
      }
      \caption*{\text{shape}}
     \end{subfigure}
     \caption{The five O2D relations. }
     \label{fig:rels}
 \end{figure}

\begin{figure}
\begin{multicols}{2}
\begin{center}\includegraphics[scale = .05]{images/blocks2.png}\end{center}
\columnbreak
\tiny
\begin{Verbatim}[gobble=4,commandchars=\\\{\}]
    \textcolor{blue}{% types}
    robot(r). table(t).
    block(b0). block(b1). 
    ...
    \textcolor{blue}{% spatial relations}
    overlaps-with(b0,r). 
    below-of(t,b1). 
    smaller-than(b1,r).
    ...
    \textcolor{blue}{% shapes}
    shape(r,rectangle). 
    shape(b0,rectangle). 
    ...
\end{Verbatim}
\end{multicols}
 \caption{A Blocksworld state: PDDLGym image and O2D state.} 
 \label{fig:blocks} 
\end{figure} 
 

